GraphWorld: Fake Graphs Bring Real Insights for GNNs

Despite advances in the field of Graph Neural Networks (GNNs), only a small number (~5) of datasets are currently used to evaluate new models. This continued reliance on a handful of datasets provides minimal insight into the performance differences between models, and is especially challenging for industrial practitioners who are likely to have datasets which look very different from those used as academic benchmarks. In the course of our work on GNN infrastructure and open-source software at Google, we have sought to develop improved benchmarks that are robust, tunable, scalable,and generalizable. In this work we introduce GraphWorld, a novel methodology and system for benchmarking GNN models on an arbitrarily-large population of synthetic graphs for any conceivable GNN task. GraphWorld allows a user to efficiently generate a world with millions of statistically diverse datasets. It is accessible, scalable, and easy to use. GraphWorld can be run on a single machine without specialized hardware, or it can be easily scaled up to run on arbitrary clusters or cloud frameworks. Using GraphWorld, a user has fine-grained control over graph generator parameters, and can benchmark arbitrary GNN models with built-in hyperparameter tuning. We present insights from GraphWorld experiments regarding the performance characteristics of tens of thousands of GNN models over millions of benchmark datasets. We further show that GraphWorld efficiently explores regions of benchmark dataset space uncovered by standard benchmarks, revealing comparisons between models that have not been historically obtainable. Using GraphWorld, we also are able to study in-detail the relationship between graph properties and task performance metrics, which is nearly impossible with the classic collection of real-world benchmarks.

==> contents/0.teaserfigure.tex <==
\begin{teaserfigure}
\centering
\includegraphics[width=.3\textwidth]{figures/distribution.png}\hfill
\includegraphics[width=.3\textwidth]{figures/gat.png}\hfill
\includegraphics[width=.3\textwidth]{figures/appnp.png}

\caption{default}
\label{fig:heatmaps}
\end{teaserfigure}


==> contents/6.acknowledgements.tex <==
\vspace{-1.5mm}
\begin{acks}
We thank Google Cloud for supporting this project.
\end{acks}

==> data/lp_aucs_tuning.tex <==
x APPNP ARMA Baseline FiLM GAT GATv2 GCN GIN GraphSAGE MLP SGC SuperGAT Transformer
1 83.48 92.46 66.83 78.27 90.59 82.20 79.12 82.54 83.73 76.81 76.39 82.27 87.86
2 80.12 92.21 66.79 78.26 80.66 80.20 79.00 81.77 80.15 76.67 76.38 80.23 79.07
3 79.62 91.96 66.74 78.26 78.80 78.64 78.89 80.99 76.57 76.52 76.38 78.45 78.39
4 79.03 88.41 66.70 78.17 78.22 78.28 78.69 80.76 75.97 76.46 76.38 78.15 78.24
5 78.76 84.45 66.66 78.07 77.50 78.01 78.48 80.58 75.92 76.44 76.37 77.96 78.20
6 78.61 83.50 66.64 78.03 77.19 77.46 78.43 80.55 75.89 76.42 76.37 77.83 78.09
7 78.28 83.36 66.63 78.02 77.01 77.42 78.43 80.55 75.88 76.40 76.34 77.72 77.99
8 78.14 83.25 66.62 77.96 76.87 77.15 78.41 80.54 75.86 76.38 76.31 77.55 77.96
9 78.03 83.16 66.61 77.86 76.77 76.94 78.38 80.54 75.84 76.36 76.27 77.49 77.92
10 77.89 82.61 66.57 77.79 76.59 76.74 78.35 80.52 75.76 76.34 76.24 77.19 77.77
11 77.80 81.73 66.52 77.78 76.52 76.07 78.32 80.50 75.60 76.31 76.20 76.24 77.61
12 77.76 81.05 66.46 77.76 76.46 76.04 78.31 80.46 75.47 76.28 76.17 76.12 77.54
13 77.68 80.58 66.41 77.72 76.42 76.01 78.30 80.42 75.41 76.25 76.16 76.10 77.52
14 77.66 80.27 66.23 77.69 76.33 75.97 78.29 80.31 75.35 76.20 76.16 76.07 77.50
15 77.62 80.24 65.98 77.69 76.15 75.91 78.29 80.15 75.34 76.17 76.16 76.03 77.44
16 77.57 80.21 65.72 77.68 76.06 75.89 78.27 80.02 75.32 76.14 76.15 75.99 77.36
17 77.53 80.20 65.46 77.68 76.00 75.88 78.25 79.91 75.27 76.12 76.13 75.96 77.35
18 77.49 80.18 65.33 77.68 75.96 75.86 78.23 79.85 75.21 76.10 76.12 75.94 77.34
19 77.45 80.17 65.31 77.66 75.93 75.84 78.21 79.83 75.14 76.08 76.11 75.92 77.33
20 77.39 80.15 65.30 77.63 75.86 75.83 78.18 79.80 75.07 76.04 76.11 75.88 77.32
21 77.32 80.12 65.28 77.62 75.81 75.81 78.13 79.76 75.04 75.99 76.10 75.83 77.31
22 77.26 80.09 65.26 77.62 75.79 75.76 78.08 79.68 75.03 75.95 76.09 75.78 77.28
23 77.22 80.01 65.24 77.59 75.74 75.76 78.07 79.54 75.01 75.93 76.09 75.76 77.25
24 77.18 79.92 65.21 77.54 75.74 75.73 78.06 79.43 74.97 75.91 76.09 75.74 77.22
25 77.13 79.88 65.18 77.50 75.73 75.65 78.05 79.37 74.94 75.72 76.09 75.68 77.18
26 77.07 79.85 65.15 77.50 75.68 75.62 78.03 79.32 74.90 75.52 76.08 75.63 77.16
27 77.03 79.81 65.15 77.47 75.65 75.61 77.98 79.28 74.86 75.39 76.08 75.58 77.09
28 76.96 79.78 65.14 77.32 75.64 75.59 77.93 79.25 74.83 75.29 76.07 75.57 77.08
29 76.91 79.76 65.13 77.18 75.64 75.55 77.90 79.23 74.79 75.18 76.00 75.57 77.01
30 76.85 79.74 65.11 77.11 75.62 75.49 77.89 79.22 74.77 75.07 75.85 75.55 76.94
31 76.81 79.71 65.08 77.05 75.58 75.42 77.85 79.21 74.74 74.96 75.71 75.52 76.93
32 76.76 79.69 65.04 76.98 75.54 75.38 77.77 79.21 74.71 74.95 75.14 75.49 76.87
33 76.74 79.67 65.00 76.91 75.52 75.31 77.68 79.21 74.67 74.94 74.43 75.45 76.84
34 76.71 79.67 64.96 76.88 75.44 75.27 77.58 79.21 74.59 74.87 73.73 75.40 76.82
35 76.65 79.66 64.95 76.85 75.30 75.27 77.50 79.20 74.49 74.79 73.68 75.39 76.78
36 76.61 79.65 64.95 76.79 75.29 75.21 77.50 79.18 74.44 74.58 73.63 75.37 76.74
37 76.57 79.64 64.94 76.72 75.28 75.17 77.48 79.18 74.43 74.24 73.58 75.33 76.73
38 76.55 79.63 64.93 76.65 75.16 75.14 77.37 79.17 74.41 73.88 73.56 75.28 76.65
39 76.50 79.62 64.52 76.56 75.05 75.13 77.27 79.12 74.38 73.45 73.54 75.25 76.51
40 76.46 79.59 64.05 76.49 75.00 75.12 77.27 79.07 74.34 73.02 73.53 75.20 76.42
41 76.43 79.56 63.58 76.45 74.96 75.09 77.27 79.05 74.30 72.83 73.51 75.16 76.39
42 76.38 79.51 63.11 76.41 74.91 75.05 77.19 79.05 74.26 72.69 73.50 75.13 76.37
43 76.35 79.46 62.83 76.31 74.87 74.99 77.10 79.03 74.23 72.61 73.32 75.08 76.36
44 76.31 79.45 62.62 76.20 74.84 74.98 77.06 79.01 74.21 72.61 73.08 75.04 76.32
45 76.25 79.44 62.41 76.14 74.76 74.87 77.04 78.98 74.12 72.58 72.85 74.98 76.24
46 76.14 79.42 62.20 76.09 74.75 74.86 76.95 78.96 74.02 72.49 72.84 74.97 76.12
47 76.09 79.39 62.09 75.93 74.65 74.83 76.86 78.95 73.97 72.41 72.83 74.96 75.99
48 76.04 79.38 62.04 75.75 74.58 74.73 76.77 78.94 73.92 72.38 72.83 74.94 75.91
49 75.97 79.37 61.99 75.66 74.48 74.70 76.68 78.93 73.68 72.36 72.82 74.89 75.88
50 75.96 79.36 61.95 75.63 74.43 74.59 76.62 78.92 73.32 72.31 72.81 74.87 75.80
51 75.89 79.35 61.91 75.58 74.36 74.56 76.56 78.89 73.10 72.25 72.78 74.75 75.75
52 75.81 79.32 61.90 75.53 74.32 74.54 76.50 78.86 73.01 72.21 72.71 74.66 75.62
53 75.76 79.27 61.88 75.48 74.28 74.46 76.44 78.83 72.92 72.19 72.65 74.52 75.49
54 75.69 79.24 61.86 75.45 74.07 74.33 76.40 78.82 72.83 72.16 72.56 74.49 75.27
55 75.62 79.22 61.83 75.43 73.92 74.26 76.39 78.77 72.73 71.98 72.48 74.43 75.15
56 75.54 79.20 61.79 75.41 73.89 73.90 76.38 78.65 72.62 71.81 72.39 74.39 75.11
57 75.49 79.18 61.75 75.38 73.74 73.73 76.36 78.56 72.50 71.75 72.34 74.36 75.11
58 75.39 79.16 61.71 75.17 73.60 73.62 76.33 78.54 72.28 71.74 72.29 74.28 75.01
59 75.36 79.15 61.67 74.95 73.57 73.26 76.17 78.52 72.07 71.67 72.25 73.97 74.98
60 75.28 79.13 61.64 74.89 73.52 73.02 76.00 78.48 72.00 71.53 72.25 73.81 74.97
61 75.23 79.06 61.61 74.85 73.44 72.99 75.85 78.45 71.94 71.37 72.25 73.75 74.96
62 75.17 78.99 61.58 74.43 73.38 72.84 75.69 78.41 71.83 71.03 72.24 73.65 74.86
63 75.08 78.97 61.54 73.89 73.35 72.67 75.33 78.37 71.69 70.68 72.22 73.57 74.74
64 75.01 78.95 61.46 73.64 73.23 72.64 74.95 78.32 71.45 70.53 72.21 73.52 74.66
65 74.91 78.91 61.37 73.62 72.96 72.46 74.82 78.27 71.15 70.41 72.18 73.34 74.52
66 74.73 78.87 61.28 73.55 72.43 72.28 74.74 78.23 70.79 70.33 72.14 73.21 74.29
67 74.68 78.75 61.20 73.43 71.88 72.21 74.67 78.19 70.37 70.28 72.11 73.14 74.24
68 74.63 78.60 61.13 73.31 71.60 72.16 74.60 78.18 70.04 70.23 72.05 73.10 74.01
69 74.59 78.37 61.06 73.19 71.46 72.14 74.57 78.18 69.94 70.17 72.00 73.04 73.69
70 74.51 78.09 61.00 73.09 71.40 72.11 74.56 78.13 69.85 70.11 71.95 72.81 73.45
71 74.43 77.90 60.93 73.08 71.33 72.02 74.53 78.07 69.81 70.10 71.87 72.71 73.36
72 74.41 77.79 60.87 73.08 71.21 71.93 74.47 78.01 69.76 70.10 71.80 72.45 73.35
73 74.27 77.71 60.82 72.88 70.99 71.88 74.39 77.94 69.70 69.34 71.76 71.83 73.24
74 74.14 77.65 60.77 72.68 70.69 71.85 74.26 77.79 69.64 68.13 71.74 71.35 73.00
75 74.05 77.55 60.72 72.56 70.42 71.82 74.13 77.61 69.55 67.29 71.72 71.27 72.90
76 73.97 77.32 60.65 72.45 70.07 71.56 74.04 77.47 69.45 67.20 71.72 71.19 72.29
77 73.89 77.04 60.57 72.38 69.94 70.96 73.93 77.34 69.37 67.11 71.72 70.96 72.17
78 73.80 76.55 60.49 72.33 69.88 70.66 73.78 77.08 69.31 67.11 71.71 70.64 72.14
79 73.73 76.09 60.41 72.21 69.78 70.32 73.64 76.77 69.14 67.11 71.70 70.38 72.04
80 73.64 76.00 60.06 72.02 69.59 69.96 73.58 76.63 68.87 66.97 71.69 69.38 71.94
81 73.58 75.91 59.55 71.76 69.45 69.88 73.52 76.61 68.51 66.78 71.67 69.10 71.84
82 73.50 75.76 59.04 71.39 68.98 69.57 73.10 76.43 67.96 66.42 71.66 69.09 71.64
83 73.34 75.62 58.53 70.89 68.71 69.25 72.66 76.15 67.53 65.81 71.64 68.56 71.44
84 73.15 75.59 58.21 69.90 68.66 69.09 72.39 75.93 67.51 65.20 71.56 68.31 71.18
85 72.96 75.58 58.10 68.97 68.56 69.05 72.16 75.78 67.48 64.64 71.40 67.79 71.13
86 72.80 75.56 57.99 68.85 68.25 68.97 71.93 75.60 67.20 64.07 71.24 67.60 70.47
87 72.62 75.54 57.88 68.73 68.21 68.85 71.70 75.40 66.93 60.91 71.18 67.29 69.76
88 72.56 75.26 57.78 66.91 68.11 68.18 71.59 75.26 66.73 57.16 71.14 67.20 69.48
89 72.24 74.83 57.69 64.92 67.40 67.72 71.54 75.23 66.55 54.96 71.10 66.96 68.83
90 72.01 74.31 57.61 63.37 67.13 67.00 71.36 75.11 65.30 54.25 71.09 66.90 68.41
91 71.78 73.71 57.53 61.96 67.10 66.13 71.06 74.76 63.72 53.58 71.08 66.80 67.83
92 71.65 73.33 57.44 61.37 65.74 65.72 70.59 74.48 62.86 53.13 71.07 66.55 67.09
93 71.37 73.25 57.33 61.30 64.91 65.34 69.91 74.37 62.46 52.67 71.06 65.36 65.52
94 70.76 72.92 57.22 60.03 63.70 63.72 69.40 74.23 61.55 52.17 71.05 64.61 64.81
95 70.07 72.07 57.11 57.33 62.25 62.44 69.22 74.02 60.03 51.67 71.02 62.77 61.24
96 69.41 71.04 57.01 55.40 61.80 62.02 68.99 73.81 58.96 50.75 70.97 61.40 60.41
97 68.87 69.31 57.01 55.26 60.46 59.75 68.54 73.59 58.91 49.54 70.92 57.72 59.95
98 67.95 67.77 57.01 55.14 58.52 58.40 68.13 73.38 58.88 48.71 70.90 56.44 59.60
99 67.30 67.77 57.01 55.14 54.42 57.08 68.13 73.38 58.88 48.71 70.90 53.98 54.63
100 62.34 67.77 57.01 55.14 53.37 56.77 68.13 73.38 58.88 48.71 70.90 53.41 53.61

==> figures/firstpage_bucketed.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={
    group name=myplot,
    group size= 1 by 2,
    horizontal sep=0.45cm,
    vertical sep=1cm},
    height=5cm,
  width=\columnwidth,
  colormap/RdYlGn,
  mesh/ordering=y varies,
  mesh/rows=30,
  unbounded coords=jump,
  zmin=0,
  zmax=1,
  point meta min=0,
  point meta max=.8,
  zlabel=Mean reciprocal rank,
  xlabel=edge homogeneity,
  ylabel=avg.\ degree,
    ]
\nextgroupplot[
]
  \addplot3[surf] table {data/kdd_bucketed/mode2_sbm_GCN.csv};
  \addplot3[surf, point meta=explicit] table [z expr=1, meta index=2] {data/kdd_bucketed/mode2_sbm_GCN.csv};
  \addplot3 [color=black, draw=none, mark=*, mark size=2]
            table[row sep=crcr] {%
            0.8138 2 1\\ % cora
            0.7461 1.42 1\\ % citeseer
            0.6551 6.89 1\\ % arxiv
            0.8024 4.50 1\\ % pubmed
            0.8076 20 1\\ % products
            };
    \node[anchor=west] at (axis cs: 0.8138,2,1) {Cora};
    \node[anchor=south east] at (axis cs: 0.7461,1.42,1) {Citeseer};
    \node[anchor=south east] at (axis cs: 0.655,6.89,1) {OGB-ArXiv};
    \node[anchor=south west] at (axis cs: 0.8024,4.50,1) {PubMed};
    \node[anchor=north east] at (axis cs: 0.8076,20,1) {OGB-Products};
    
\nextgroupplot[
colorbar horizontal,
]
  \addplot3[surf] table {data/kdd_bucketed/mode2_sbm_FiLM.csv};
  \addplot3[surf, point meta=explicit] table [z expr=1, meta index=2] {data/kdd_bucketed/mode2_sbm_FiLM.csv};
  \addplot3 [color=black, draw=none, mark=*, mark size=2]
            table[row sep=crcr] {%
            0.8138 2 1\\ % cora
            0.7461 1.42 1\\ % citeseer
            0.6551 6.89 1\\ % arxiv
            0.8024 4.50 1\\ % pubmed
            0.8076 20 1\\ % products
            };
    \node[anchor=west] at (axis cs: 0.8138,2,1) {Cora};
    \node[anchor=south east] at (axis cs: 0.7461,1.42,1) {Citeseer};
    \node[anchor=south east] at (axis cs: 0.655,6.89,1) {OGB-ArXiv};
    \node[anchor=south west] at (axis cs: 0.8024,4.50,1) {PubMed};
    \node[anchor=north east] at (axis cs: 0.8076,20,1) {OGB-Products};
\end{groupplot}
\end{tikzpicture}   
\caption{Please add caption.\label{fig:my_label}}
\end{figure}

==> figures/mode2_combined.tex <==
\begin{figure*}[htb]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={
    group name=myplot,
    group size= 4 by 2,
    horizontal sep=0.45cm,
    vertical sep=0.45cm},
    height=5cm,
    width=0.29\linewidth,
    title style={at={(0.5,0.97)},anchor=south},
    every axis x label/.style={at={(axis description cs:0.5,-0.1)}, anchor=north},
    every axis y label/.style={at={(axis description cs:-0.15,0.5)}, anchor=south, rotate=90},
    legend image code/.code={
    \draw
    plot coordinates {
    (0cm,0cm)
    (0.475cm,0cm)         %% default is (0.6cm,0cm)
    };%
    }
    ]
\nextgroupplot[
 	%title = \textbf{Meow},
 	legend columns=12,
	legend style={at={(2.25,1.05)},anchor=south},
    ylabel style={align=center},
	ylabel={Node classification \\ ROC AUC$\times100$},
	xmin=1,
	xmax=10,
	ymin=50,
	ymax=100,
    ytick={50,60,70,80,90,100},
	%xtick=\empty,
    legend entries={GCN, GIN, GAT, GraphSAGE, APPNP, SGC, ARMA, GATv2, FiLM, MLP, Baseline},
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};
\addplot[very thick,color=cycle11] table[x=x,y=PPRBaseline_mean] {data/25/mode2_sbm_p_to_q_ratio.csv};

\nextgroupplot[
 	%title = \textbf{Meow},
	xmin=0,
	xmax=5,
	ymin=50,
	ymax=100,
	%xtick=\empty,
	ytick=\empty,
    xtick={0,2,4,5},
]

\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_sbm_feature_center_distance.csv};
\addplot[very thick,color=cycle11] table[x=x,y=PPRBaseline_mean] {data/25/mode2_sbm_feature_center_distance.csv};

\nextgroupplot[
 	%title = \textbf{Meow},
	xmin=1,
	xmax=20,
	ymin=50,
	ymax=62,
	%xtick=\empty,
	xshift=0.45cm,
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_sbm_avg_degree.csv};
\addplot[very thick,color=cycle11] table[x=x,y=PPRBaseline_mean] {data/25/mode2_sbm_avg_degree.csv};

\nextgroupplot[
 	%title = \textbf{Meow},
	xmin=128,
	xmax=512,
	ymin=50,
	ymax=62,
	%xtick=\empty,
	ytick=\empty,
]

\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_sbm_nvertex.csv};
\addplot[very thick,color=cycle11] table[x=x,y=PPRBaseline_mean] {data/25/mode2_sbm_nvertex.csv};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[
 	%title = \textbf{Meow},
    ylabel style={align=center},
	ylabel={Link prediction \\ ROC AUC$\times100$},
	xlabel=\nicefrac{p}{q} ratio,
	xmin=1,
	xmax=10,
	ymin=58,
	ymax=85,
    ytick={60,70,80,85},
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\addplot[very thick,color=cycle11] table[x=x,y=Baseline_mean] {data/25/mode2_lp_p_to_q_ratio.csv};
\nextgroupplot[
 	%title = \textbf{Meow},
	xlabel=feature center distance,
	xmin=0,
	xmax=5,
	ymin=58,
	ymax=85,
	ytick=\empty,
    xtick={0,2,4,5},
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_lp_feature_center_distance.csv};
\addplot[very thick,color=cycle11] table[x=x,y=Baseline_mean] {data/25/mode2_lp_feature_center_distance.csv};
\nextgroupplot[
 	%title = \textbf{Meow},
	xlabel=avg.\ degree,
	xmin=1,
	xmax=20,
	ymin=50,
	ymax=85,
    ytick={50,60,70,80,85},
    xtick={0,5,10,15,20},
	%xshift=0.75cm,
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_lp_avg_degree.csv};
\addplot[very thick,color=cycle11] table[x=x,y=Baseline_mean] {data/25/mode2_lp_avg_degree.csv};
\nextgroupplot[
 	%title = \textbf{Meow},
	xlabel=$n$,
	xmin=128,
	xmax=512,
	ymin=50,
	ymax=85,
	ytick=\empty,
]
\addplot[very thick,color=cycle1] table[x=x,y=GCN_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle2] table[x=x,y=GIN_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle3] table[x=x,y=GAT_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle4] table[x=x,y=GraphSAGE_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle5] table[x=x,y=APPNP_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle6] table[x=x,y=SGC_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle7] table[x=x,y=ARMA_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle8] table[x=x,y=GATv2_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle9] table[x=x,y=FiLM_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle10] table[x=x,y=MLP_mean] {data/25/mode2_lp_nvertex.csv};
\addplot[very thick,color=cycle11] table[x=x,y=Baseline_mean] {data/25/mode2_lp_nvertex.csv};
\end{groupplot}
\end{tikzpicture}
\caption{Node classification and link prediction results from a fixed default parameter set.}\label{fig:synthetic-results-pooling}
\end{figure*}

==> keywords.tex <==
%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
%\begin{CCSXML}
%<ccs2012>
% <concept>
%  <concept_id>10010520.10010553.10010562</concept_id>
%  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
%  <concept_significance>500</concept_significance>
% </concept>
% <concept>
%  <concept_id>10010520.10010575.10010755</concept_id>
%  <concept_desc>Computer systems organization~Redundancy</concept_desc>
%  <concept_significance>300</concept_significance>
% </concept>
% <concept>
%  <concept_id>10010520.10010553.10010554</concept_id>
%  <concept_desc>Computer systems organization~Robotics</concept_desc>
%  <concept_significance>100</concept_significance>
% </concept>
% <concept>
%  <concept_id>10003033.10003083.10003095</concept_id>
%  <concept_desc>Networks~Network reliability</concept_desc>
%  <concept_significance>100</concept_significance>
% </concept>
%</ccs2012>
%\end{CCSXML}

%\ccsdesc[500]{Computer systems organization~Embedded systems}
%\ccsdesc[300]{Computer systems organization~Redundancy}
%\ccsdesc{Computer systems organization~Robotics}
%\ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
% Taking too much space now, let's do them in the camera-ready – A 15.10
%% the work being presented. Separate the keywords with commas.
%\keywords{graphs, graph neural networks, benchmark}


==> tables/insights-table.tex <==
\begin{table*}[t]
\centering
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{tabularx}{\linewidth}{CCCCCCCC}
\toprule
\multicolumn{2}{c}{\emph{model}} & \multicolumn{6}{c}{\emph{parameter}} \\
\emph{name} & \emph{type} & \nicefrac{p}{\!q} ratio & feature center dist & avg degree & n nodes & cluster size slope& power exponent\\
\godownup & \gostraight & \gostraight & \gostraight & \gostraight & \gostraight \\
 \goup & \gostraight & \gostraight & \goup & \gostraight & \goup & \gostraight & \gostraight & \godown
 \goup & \gostraight & \godown & \gostraight & \gostraight & \gostraight & \gostraight \\
 \goup & \gostraight & \gostraight & \gostraight & \gostraight & \gostraight \\
 & \gostraight & \gostraight & \gostraight & \gostraight & \gostraight & \godown  \\
 \goup & \gostraight & \gostraight & \goup & \gostraight & \goup & \gostraight & \gostraight & \godown  \\
 & \gostraight & \godown & \gostraight & \goup & \gostraight & \goup & \gostraight & \gostraight & \godown  \\
 \goup & \gostraight & \godown & \gostraight & \gostraight & \gostraight & \gostraight  \\
 \goup & \gostraight & \godown & \gostraight & \gostraight & \gostraight & \gostraight  \\
 \goup & \gostraight & \gostraight & \gostraight & \gostraight & \gostraight  \\
 \goup & \gostraight & \gostraight & \goup & \gostraight & \godown & \gostraight & \gostraight & \godown  \\
\bottomrule
\end{tabularx}
\caption{Model performance insights: what is good and what is not}
\label{tab:insights}
\end{table*}
